Concrete resource analysis of the quantum linear system algorithm used to compute the electromagnetic scattering cross section of a 2D target

We provide a detailed estimate for the logical resource requirements of the quantum linear system algorithm (QLSA) [Phys. Rev. Lett. 103, 150502 (2009)] including the recently described elaborations [Phys. Rev. Lett. 110, 250504 (2013)]. Our resource estimates are based on the standard quantum-circuit model of quantum computation; they comprise circuit width, circuit depth, the number of qubits and ancilla qubits employed, and the overall number of elementary quantum gate operations as well as more specific gate counts for each elementary fault-tolerant gate from the standard set {X, Y, Z, H, S, T, CNOT}. To perform these estimates, we used an approach that combines manual analysis with automated estimates generated via the Quipper quantum programming language and compiler. Our estimates pertain to the example problem size N=332,020,680 beyond which, according to a crude big-O complexity comparison, QLSA is expected to run faster than the best known classical linear-system solving algorithm. For this problem size, a desired calculation accuracy 0.01 requires an approximate circuit width 340 and circuit depth of order $10^{25}$ if oracle costs are excluded, and a circuit width and depth of order $10^8$ and $10^{29}$, respectively, if oracle costs are included, indicating that the commonly ignored oracle resources are considerable. In addition to providing detailed logical resource estimates, it is also the purpose of this paper to demonstrate explicitly how these impressively large numbers arise with an actual circuit implementation of a quantum algorithm. While our estimates may prove to be conservative as more efficient advanced quantum-computation techniques are developed, they nevertheless provide a valid baseline for research targeting a reduction of the resource requirements, implying that a reduction by many orders of magnitude is necessary for the algorithm to become practical.

==> results-new.tex <==
\section{Results}
\label{Sec:Results} 

\subsection{Logical resource estimate --- summary}
Our LRE for QLSA for problem size
$N=332,020,680$ is summarized in Table
\ref{TableForN=332020680}. 

\begin{table}[h!]
\begin{tabular}{|l||c|c||} \hline\hline
Resources & incl.\ oracles & excl.\ oracles  \\  \hline\hline
Max. overall number of qubits & $3\times 10^8 $ & $341$ \\ 
in use at a time & & \\ \hline
%Number of data qubits & 180& 180\\ \hline
Max. number of data & 60 & 60\\
qubits at a time & & \\ \hline
Max. number of ancilla & $3\times 10^8 $&$281$ \\ qubits in use at a time      	
 & & \\ \hline
Overall number of   ancilla    & $2.8\times 10^{27}$ & $8.2\times 10^{21}$\\                           
 generation-use-termination cycles   &	& \\ \hline
Total number of gates	&$2.37\times 10^{29}$ & $3.36\times 10^{25}$\\ \hline
\# $H$ gates	&$2.7\times 10^{28}$ & $1.20\times 10^{25}$\\ \hline
\# $S$ gates	&$1.4\times 10^{28}$ & $6.8\times 10^{24}$\\ \hline
\# $T$ gates	&$9.5\times 10^{28}$ & $1.29\times 10^{25}$\\ \hline
\# $X$ gates	&$1.6\times 10^{28}$ & $2\times 10^{23}$\\ \hline
\# CNOT gates	&$8.5\times 10^{28}$ & $1.7\times 10^{24}$\\ \hline
Circuit Width 	&	$3\times 10^{8}$ & $341$\\ \hline
Circuit Depth	&	$1.8\times 10^{29}$ & $3.32 \times 10^{25} $\\ \hline	
T-Depth		&	$8.2\times 10^{28}$ & $1.28 \times 10^{25} $\\ \hline	
Measurements 	&	$2.8\times 10^{27}$ & $8.23 \times 10^{21} $\\ \hline\hline
\end{tabular}
\caption{\label{TableForN=332020680}QLSA resource requirements for problem size $N=332,020,680$ 
and algorithmic accuracy $\epsilon=0.01$. }
\end{table}

The following subsection \label{SubSec:Results}
remarks explain this table. We discuss the results in 
Sec.~\ref{Sec:Discussion}.


\subsection{Assumptions and comments}
Unlike with QEC protocols where the distinction between 
\lq{}data qubits\rq{} and \lq{}ancilla qubits\rq{} is clear, 
here this distinction is somewhat ambiguous; indeed, 
all qubits involved in the algorithm are initially prepared 
in state $\ket{0}$, and some qubits that we called ancilla 
qubits exist from the start to the end of a full quantum 
computation part (such as e.g single-qubit registers $R_6,\: R_8$).  
We regard qubits which carry the data 
of the linear system problem and store 
its solution at the end of the quantum computation 
as data qubits; they constitute the quantum data 
registers $R_2$ and $R_3$, see Table~\ref{RegisterDefinition}. 
All other qubits, including those of QAE and HS control registers $R_0$ and $R_1$ 
as well as of the computational registers $R_4$ and $R_5$, 
are considered ancilla qubits.

It is important to note that the overall QLS algorithm consists of {\em four} 
independent quantum computation parts, namely the four calls of 
{\em \lq{}AmpEst\rq{}} subalgorithms, see Fig.~\ref{fig:QLSA-Profiling}, 
while the top-level function \lq{}{\em QLSA\_main}\rq{} performs  
a classical calculation of  the RCS (by Eq.~(\ref{Eq:RCS})) using the results 
$\phi_b$, $\phi_x$, $\phi_{r0}$, $\phi_{r1}$ of its four quantum 
computation parts. These four 
independent \lq{}AmpEst\rq{} subalgorithms can either be performed 
in parallel or sequentially, and the actual choice should be subject to any 
time/space tradeoff considerations.
Here we assume a sequential 
implementation, so that data and ancilla qubits can 
be reused by the four amplitude estimation parts. 
Hence, the qubit counts provided in Table~\ref{TableForN=332020680} 
represent the maximum number of qubits in use at a time 
required by the most demanding of the four independent \lq{}AmpEst\rq{} subalgorithms.
The maximum overall number of qubits (data and ancilla) in use at a time  
is also the definition for {\em circuit width}. While with a sequential 
implementation we aim at minimizing the circuit width (space consumption), 
we can do so only at the cost of increasing the circuit depth (time consumption). 
The overall circuit depth is the sum of the depths of the four \lq{}AmpEst\rq{} 
subalgorithms. By a brief look at Fig.~\ref{fig:QLSA-Profiling} it is clear that the 
circuit depths are similarly large for \lq{}AmpEst\_${\phi_x}$\rq{} and \lq{}AmpEst\_${\phi_r}$\rq{} 
(where the latter is called twice), whereas compared to these the circuit depth of \lq{}AmpEst\_${\phi_b}$\rq{} is negligible. Hence the overall  circuit depth is rougly 
three times the circuit depth of subalgorithm \lq{}AmpEst\_${\phi_r}$\rq{}. 
We could just as well assume a parallel implementation of the four \lq{}AmpEst\rq{} 
calls. In this case the overall circuit depth would be by a factor $1/3$ smaller than 
in the former case. However, this circuit-depth decrease can only be achieved 
at the cost of incuring a circuit-width increase.  We would need up to four copies 
of the quantum registers listed in Table~\ref{RegisterDefinition}, and  the required 
number of data and ancilla qubits in use at a time would be larger by a factor that is somewhat 
smaller than four. 

QLSA has numerous iterative operations (in particular due to
Suzuki-Higher-Order Integrator method with Trotterization) involving
ancilla qubit {\em \lq{}generation-use-termination\rq{} cycles}, which are
repeated, over and over again, while computation is performed 
on the same end-to-end data qubits. Table \ref{TableForN=332020680} 
provides an estimate for both the number of ancilla
qubits employed at a time and for the overall number of ancilla
generation-use-termination cycles executed during the 
implementation of all the four \lq{}AmpEst\rq{} subalgorithms.
To illustrate the difference we note 
that, for some quantum computer realizations, the physical information 
carriers (carrying the ancilla qubits) can be reused, for others however, 
such as photon-based quantum computer realizations,
the information carriers are lost and have to be created anew.

Furthermore, the gate counts actually mean the number of elementary
logical {\em gate operations}, independent of whether these 
operations are performed using the same physical resources (lasers,
interaction region, etc.) or not.  The huge number of measurements
results from the vast overall number of ancilla-qubit uses; after each
use an ancilla has to be uncomputed and eventually terminated to
ensure reversibility of the circuit. Finally,
Table~\ref{TableForN=332020680}  distinguishes
between the overall LRE that includes the oracle implementation and
the LRE for the bare algorithm with oracle calls regarded as
\lq{}for free\rq{} (excluding their resource requirements).



% \begin{table}[htbp]
% \begin{tabular}{|l||c|c||} \hline\hline
% Resources & incl.\ oracles & excl.\ oracles  \\  \hline\hline
% Number of data qubits & 107& 107\\ \hline
% Max. number of data & 31 & 31\\
% qubits at a time & & \\ \hline
% Overall number of   ancilla    & $2.8\times 10^{27}$ & $7.2\times 10^{21}$\\  
% generation-use-termination cycles   &	& \\ \hline
% Max. number of ancilla & $3\times 10^8 $&$262$ \\ qubits at a time      	
%  & & \\ \hline
% Total number of gates	&$2.37\times 10^{29}$ & $3.13\times 10^{25}$\\ \hline
% \# $H$ gates	&$2.7\times 10^{28}$ & $1.17\times 10^{25}$\\ \hline
% \# $S$ gates	&$1.4\times 10^{28}$ & $6.0\times 10^{24}$\\ \hline
% \# $T$ gates	&$9.5\times 10^{28}$ & $1.24\times 10^{25}$\\ \hline
% \# $X$ gates	&$1.6\times 10^{28}$ & $4.3\times 10^{22}$\\ \hline
% \# CNOT gates	&$8.5\times 10^{28}$ & $1.2\times 10^{24}$\\ \hline
% Circuit Width 	&	$3\times 10^{8}$ & $293$\\ \hline
% Circuit Depth	&	$1.8\times 10^{29}$ & $3.13 \times 10^{25} $\\ \hline	
% T-Depth		&	$8.2\times 10^{28}$ & $1.24 \times 10^{25} $\\ \hline	
% Measurements 	&	$2.8\times 10^{27}$ & $7.17 \times 10^{21} $\\ \hline\hline
% \end{tabular}
% \caption{\label{TableForN=24}Resource requirements for problem size $N=24$}
% \end{table}







